Online Domain Adaptation for Continuous Cross-Subject Liver Viability Evaluation Based on Irregular Thermal Data

Accurate evaluation of liver viability during its procurement is a challenging issue and has traditionally been addressed by taking invasive biopsy on liver. Recently, people have started to investigate on the non-invasive evaluation of liver viability during its procurement using the liver surface thermal images. However, existing works include the background noise in the thermal images and do not consider the cross-subject heterogeneity of livers, thus the viability evaluation accuracy can be affected. In this paper, we propose to use the irregular thermal data of the pure liver region, and the cross-subject liver evaluation information (i.e., the available viability label information in cross-subject livers), for the real-time evaluation of a new liver's viability. To achieve this objective, we extract features of irregular thermal data based on tools from graph signal processing (GSP), and propose an online domain adaptation (DA) and classification framework using the GSP features of cross-subject livers. A multiconvex block coordinate descent based algorithm is designed to jointly learn the domain-invariant features during online DA and learn the classifier. Our proposed framework is applied to the liver procurement data, and classifies the liver viability accurately.

==> 5_discussions.tex <==
In this research, an online domain adaptation algorithm is developed and applied to predict the viability of the harvested livers based on the features obtained from their infrared images. As mentioned in Section \ref{sec: data_collection}, these livers were preserved in different Machine Perfusion conditions and had different sizes. 

When there is not any domain adaptation (offline and online SVM), the accuracy ranges from 0.72 to 0.99 for Offline SVM (with an average of 0.80) and from 0.72 to 1.00 for Online SVM (with an average of 0.79). On average, the recalls associated with Offline and Online SVM are 0.38 and 0.25, respectively. In both methods, there are cases in which NaN values are reported for precision because no livers are classified as viable in those cases. We attribute the low classification performance of two methods to the different sizes and perfusion conditions of livers. However, it can be noted that normalization in Offline SVM can slightly mitigate the liver-to-liver variation.

When the heterogeneity is addressed by DA, the accuracy ranges from 0.79 to 0.96 (with an average of 0.88) for our algorithm, from 0.74 to 0.94 (with an average of 0.82) for Online SA and from 0.81 to 1.00 (with an average of 0.91) for Offline SA. Considering accuracy, precision and recall, our algorithm outperforms its online counterpart (Online SA) in accuracy and recall and shows a lower precision compared to Online SA; however, its superiority in recall is by far. 

Firstly, we attribute the superiority of DA methods over offline and online SVM to the fact that DA methods relax the assumption that source and target data are drawn from identical distributions.

Secondly, our algorithm owes it superiority over Online SA to the following advantages: 

\begin{itemize}
    \item Our proposed method uses Block Coordinate Proximal Descent optimization to jointly learn the domain-invariant features and classifiers, whereas SA learns subspaces and classifiers in a two-stage procedure.
    \item To regularize learning and improve performance, we use a loss function to assert that the mapping matrix changes slowly in time.
\end{itemize}

Although our algorithm does not perform as good SA applied to the idealistic and unrealistic scenario of offline prediction, it demonstrates a close performance when compared to Offline SA.


